On the Provable Advantage of Unsupervised Pretraining

Unsupervised pretraining, which learns a useful representation using a large amount of unlabeled data to facilitate the learning of downstream tasks, is a critical component of modern large-scale machine learning systems. Despite its tremendous empirical success, the rigorous theoretical understanding of why unsupervised pretraining generally helps remains rather limited -- most existing results are restricted to particular methods or approaches for unsupervised pretraining with specialized structural assumptions. This paper studies a generic framework, where the unsupervised representation learning task is specified by an abstract class of latent variable models $\Phi$ and the downstream task is specified by a class of prediction functions $\Psi$. We consider a natural approach of using Maximum Likelihood Estimation (MLE) for unsupervised pretraining and Empirical Risk Minimization (ERM) for learning downstream tasks. We prove that, under a mild ''informative'' condition, our algorithm achieves an excess risk of $\tilde{\mathcal{O}}(\sqrt{\mathcal{C}_\Phi/m} + \sqrt{\mathcal{C}_\Psi/n})$ for downstream tasks, where $\mathcal{C}_\Phi, \mathcal{C}_\Psi$ are complexity measures of function classes $\Phi, \Psi$, and $m, n$ are the number of unlabeled and labeled data respectively. Comparing to the baseline of $\tilde{\mathcal{O}}(\sqrt{\mathcal{C}_{\Phi \circ \Psi}/n})$ achieved by performing supervised learning using only the labeled data, our result rigorously shows the benefit of unsupervised pretraining when $m \gg n$ and $\mathcal{C}_{\Phi\circ \Psi} > \mathcal{C}_\Psi$. This paper further shows that our generic framework covers a wide range of approaches for unsupervised pretraining, including factor models, Gaussian mixture models, and contrastive learning.

==> counter_example.tex <==
\section{Failure of Two-Phase MLE}\label{counter_example}
Given unlabeled data $\{x_i\}^m_{i=1}$ and labeled data $\{x_j,y_j\}^n_{j=1}$, another natural scheme is to use a two-phase MLE (Algorithm \ref{mle+mle}). To be specific, in the first phase, we use MLE to estimate $\phi^* $ based on the unlabeled data $\{x_i\}^m_{i=1}$. In the second phase, we use MLE again to estimate $\psi^* $ based on pretrained $\hat\phi$ and the labeled data $\{x_j,y_j\}^{n}_{j=1}$.

% \$
% \hat\phi\leftarrow\argmax_{\phi\in\Phi}\sum^m_{i=1}\log p_{\phi}(x_i).
% \$
% In the second phase, we fix $\hat\phi$ learned in the first phase and estimate $\psi^* $ by $\hat\psi$ using data $\{x_j,y_j\}^n_{j=1}$ via MLE, i.e
% \$
% \hat\psi\leftarrow\argmax_{\psi\in\Psi}\sum^n_{j=1}\log p_{\hat\phi,\psi}(x_j,y_j).
% \$

\begin{algorithm}[H]
\caption{Two-phase MLE}\label{mle+mle}
\begin{algorithmic}[1]
\State {\bf Input:} $\{x_i\}^m_{i=1}$, $\{(x_j,y_j)\}^n_{j=1}$
\State Use unlabeled data $\{x_i\}^m_{i=1}$ to learn $\hat\phi$ via MLE:
\$
\hat\phi\leftarrow\argmax_{\phi\in\Phi}\sum^m_{i=1}\log p_{\phi}(x_i).
\$
\State Fix $\hat\phi$ and use labeled data $\{(x_j,y_j)\}^n_{j=1}$ to learn $\hat\psi$ via MLE:
\$
\hat\psi\leftarrow\argmax_{\psi\in\Psi}\sum^n_{j=1}\log p_{\hat\phi,\psi}(x_j,y_j).
\$
\State {\bf Output:} $\hat\phi$ and $\hat\psi$.
\end{algorithmic}
\end{algorithm}


Note that the two-phase MLE does not directly associate the learning process with the loss function. Thus, the only way to evaluate the prediction error is to study the total variation distance between $\P_{\hat\phi, \hat\psi}(x,y)$ and $\P_{\phi^* ,\psi^* }(x,y)$. In the pretraining phase, MLE guarantees that the estimator $\mathbb{P}_{\hat{\phi}}$ is close to $\mathbb{P}_{\phi^{*}}$ in the sense of total variation distance (Theorem \ref{tv_mle}). However, it's still possible that for some $x$, $\mathbb{P}_{\hat{\phi}}(x)=0$ while $\mathbb{P}_{\phi^{*}}(x) \neq 0$. This phenomenon may result in $\log p_{\hat\phi,\psi^* }(x_j,y_j)=-\infty$ for some labeled data in the learning of downstream tasks, which will dramatically influence the behaviour of MLE for estimating $\psi^{*}$ and finally lead to the failure of the second phase. Inspired by this idea, we give the following theorem.



\begin{theorem}\label{counter}
There exists $\Phi, \Psi, \phi^{*}\in{\Phi}, \psi^{*}\in{\Psi}$, such that for any constant $c>0$, there exists $m,n \geq c$ such that with probability at least $\frac{1}{2}(1-e^{-1})e^{-1}$, we have
\$
\TV\big(\P_{\hat\phi,\hat\psi}(x,y),\P_{\phi^* ,\psi^* }(x,y)\big)\geq \frac{1}{8},
\$
where $\hat\phi$ and $\hat\psi$ are the outputs of Algorithm \ref{mle+mle}.
\end{theorem}


% Here we briefly explain why Algorithm \ref{mle+mle} may fail under some circumstances. In the first phase, MLE guarantees that the estimator $\mathbb{P}_{\hat{\phi}}$ is close to $\mathbb{P}_{\phi^{*}}$ under total variation distance (Theorem \ref{tv_mle}). But it's still possible that for some $x$, $\mathbb{P}_{\hat{\phi}}(x)=0$ while $\mathbb{P}_{\phi^{*}}(x) \neq 0$, which results in $\log\mathbb{P}_{\hat{\phi}}(x)=\log 0 = -\infty$. This phenomenon will dramatically influence the behaviour of MLE for estimating $\psi^{*}$ and will finally lead to the failure of the second phase.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> preliminaries.tex <==
\section{Preliminaries}
\noindent\textbf{Notation:} We denote by $\P(x)$ and $p(x)$ the cumulative distribution function and the probability density function defined on $x\in\mathcal{X}$, respectively. We define $[n]=\{1,2,\ldots,n\}$. The cardinality of set $\mathcal{A}$ is denoted by $|\mathcal{A}|$. Let $\|\cdot\|_2$ be the $\ell_2$ norm of a vector or the spectral norm of a matrix. We denote by $\|\cdot\|_{\rF}$ the Frobenius norm of a matrix. For a matrix $M\in\R^{m\times n}$, we denote by $\sigma_{\min}(M)$ and $\sigma_{\max}(M)$ the smallest non-zero singular value and the largest singular value of $M$, respectively. 


% We use $\tilde{\mathcal{O}}(\cdot)$ and $\tilde{\Omega}(\cdot)$ notation to hide polylogarithmic factors. The use of $\mathcal{O}$, $\Omega$ and $\Theta$ is standard.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Basic Definitions}

To measure the difference between two probability distributions, we give the formal definition of the total variation distance and the Hellinger Distance as follows. 
\begin{definition}[Total Variation Distance and Hellinger Distance]\label{def_tv}
Suppose that $\P_1$ and $\P_2$ are two probability measures defined on a measurable space $(\mathcal{X},\mathcal{F})$. The total variation distance between $\P_1$ and $\P_2$ is defined as,
\$
\TV(\P_1,\P_2):=\sup_{A\in\mathcal{F}}|\P_1(A)-\P_2(A)|.
\$
Let $\mu$ be a measure defined on $(\mathcal{X},\mathcal{F})$ such that $\P_1\ll\mu$, $\P_2\ll\mu$. It then holds that
\$
\TV(\P_1,\P_2)=\frac{1}{2}\int_{\mathcal{X}} |p_1-p_2|\, d\mu.
\$
Here 
\$
p_1:=\frac{d\P_1}{d\mu},\quad p_2:=\frac{d\P_2}{d\mu}.
\$
The square of Hellinger distance between $\P_1$ and $\P_2$ is defined as
\$
H^2(\P_1,\P_2)=\frac{1}{2}\int_{\mathcal{X}}(\sqrt{p_1}-\sqrt{p_2})^2\,d\mu.
\$
\end{definition}

Note that if $\mathcal{X}\subset\R^d$, then $p_1$ and $p_2$ are the probability density functions of the cumulative distributions $\P_1$ and $\P_2$. In the following, we focus on the case where $\mathcal{X}\subset\R^{d}$. We denote by $\mP_{\mathcal{X}}(\Phi)$ a set of parameterized density functions $p_{\phi}(x)$ defined on $x\in\mathcal{X}$
\$
\mP_{\mathcal{X}}(\Phi):=\{p_{\phi}(x)\,|\,\phi\in\Phi\},
\$
where $\phi\in\Phi$ is the parameter. Our main results will be phrased in terms of bracketing number for the class $\mP_{\mathcal{X}}(\Phi)$ under $\|\cdot\|_1$ distance, which is defined as follows.


\begin{definition}[$\epsilon$-Bracket and Bracketing Number]
Let $\epsilon>0$. Under $\|\cdot\|_1$ distance, a set of functions $\mN_{\b}(\mP_{\mathcal{X}}(\Phi),\epsilon)$ is an $\epsilon$-bracket of $\mP_{\mathcal{X}}(\Phi)$ if for any $p_{\phi}(x)\in\mP_{\mathcal{X}}(\Phi)$, there exists a function $\bar p_{\phi}(x)\in\mN_{\b}(\mP_{\mathcal{X}}(\Phi),\epsilon)$ such that the following two properties hold:
\begin{itemize}
    \item $\bar p_{\phi}(x)\geq p_{\phi}(x),~\forall x\in\mathcal{X}$
    \item $\|\bar p_{\phi}(x)-p_{\phi}(x)\|_1=\int |\bar p_{\phi}(x)- p_{\phi}(x)|\, dx\leq \epsilon$
\end{itemize}
Note that $\bar p_{\phi}(x)$ need not to belong to $\mP_{\mathcal{X}}(\Phi)$. The bracketing number $N_{\b}(\mP_{\mathcal{X}}(\Phi),\epsilon)$ is the cardinality of the smallest $\epsilon$-bracket needed to cover $\mP_{\mathcal{X}}(\Phi)$. The entropy is defined as the logarithm of the bracketing number.
\end{definition}

To measure the complexity of a function class, we consider the Rademacher complexity defined as follows.
\begin{definition}[Rademacher Complexity]
Suppose that $x_1,\ldots,x_n$ are sampled i.i.d from a probability distribution defined on a set $\mathcal{X}$. Let $\mathcal{G}$ be a class of functions mapping from $\mathcal{X}$ to $\R$. The empirical Rademacher complexity of $\mathcal{G}$ is defined as follows,
\$
\hat R_n(\mathcal{G}):=\E_{\sigma_i}\bigg[\sup_{g\in\mathcal{G}}\frac{2}{n}\sum^{n}_{i=1}\sigma_i g(x_i)\bigg],
\$
where $\{\sigma_i\}^n_{i=1}$ are independent random variables drawn from the Rademacher distribution and the expectation is taken over the randomness of $\{\sigma_i\}^n_{i=1}$. The Rademacher complexity of $\mathcal{G}$ is defined as
\$
R_n(\mathcal{G}):=\E_{x_i}[\hat R_n(\mathcal{G})],
\$
where the expectation is taken over the randomness of samples $\{x_i\}^n_{i=1}$.
\end{definition}



==> proof_contrastive_hellinger.tex <==
\subsection{Hellinger Distance Guarantee}\label{hellinger_guarantee}
Suppose that $\hat\theta$ is the output of Algorithm \ref{mle+erm}, which satisfies 
\%
\hat\theta\leftarrow \argmax_{\theta\in\Theta}\sum^{m}_{i=1}\log p_{f_{\theta}}(x_i,x'_{i},t_i).
\%
We have the following theoretical guarantee on the Hellinger distance between $\P_{f_{\hat\theta}}(x,x',t)$ and $\P_{f_{\theta^* }}(x,x',t)$.
\begin{lemma}\label{mle_hellinger}
Let $\hat\theta$ be the output of Algorithm \ref{mle+erm}. It then holds that with probability at least $1-\delta$ that
\%
H\big(\P_{f_{\hat\theta}}(x,x',t),\P_{f_{\theta^* }}(x,x',t)\big)\leq \sqrt{\frac{2}{m}\log\frac{N_{\b}\big(\mP(\mathcal{F}_{\theta}),1/m^2\big)}{\delta}},
\%
where we define $\mP(\mathcal{F}_{\theta}):=\{p_{f_{\theta}}(x,x',t)\,|\,\theta\in\Theta\}$.
\end{lemma}
\begin{proof}[Proof of Lemma \ref{mle_hellinger}]
For notation simplicity, we denote $\bm{x}:=(x,x',t)$. Let $\epsilon>0$. Similar to the proof of Theorem \ref{tv_mle}, we obtain with probability at least $1-\delta$
\%\label{101508}
1-\int\sqrt{\bar{p}_{f_{\hat\theta}}(\bm{x})p_{f_{\theta^* }}(\bm{x})}\,d\bm{x}\leq \frac{1}{m}\log\frac{N_{\b}\big(\mP(\mathcal{F}_{\theta}),\epsilon\big)}{\delta}.
\%
Here $\bar{p}_{f_{\hat\theta}}(\bm{x})\in\mN_{\b}(\mP(\mathcal{F}_{\theta}),\epsilon)$ that satisfies $\bar{p}_{f_{\hat\theta}}(\bm{x})\geq p_{f_{\hat\theta}}(\bm{x})$ for any $\bm{x}$ and 
\%
\int \bar{p}_{f_{\hat\theta}}(\bm{x})-p_{f_{\hat\theta}}(\bm{x})\,d\bm{x}\leq \epsilon.
\%
Note that
\%\label{101509}
&1-\int\sqrt{{p}_{f_{\hat\theta}}(\bm{x})p_{f_{\theta^* }}(\bm{x})}\,d\bm{x}-\bigg(1-\int\sqrt{\bar{p}_{f_{\hat\theta}}(\bm{x})p_{f_{\theta^* }}(\bm{x})}\,d\bm{x}\bigg)\notag\\
&=\int\Big(\sqrt{\bar{p}_{f_{\hat\theta}}(\bm{x})}-\sqrt{{p}_{f_{\hat\theta}}(\bm{x})}\Big)\sqrt{{p}_{f_{\theta^* }}(\bm{x})}\,d\bm{x}\notag\\
&\leq \sqrt{\int\Big(\sqrt{\bar{p}_{f_{\hat\theta}}(\bm{x})}-\sqrt{{p}_{f_{\hat\theta}}(\bm{x})}\Big)^2\,d\bm{x}}\notag\\
&=\sqrt{\int \bar{p}_{f_{\hat\theta}}(\bm{x})+{p}_{f_{\hat\theta}}(\bm{x})-2\sqrt{\bar{p}_{f_{\hat\theta}}(\bm{x}){p}_{f_{\hat\theta}}(\bm{x})} \,d\bm{x}}\notag\\
&\leq \sqrt{\int \bar{p}_{f_{\hat\theta}}(\bm{x})-{p}_{f_{\hat\theta}}(\bm{x})\,d\bm{x}}\notag\\
&\leq \sqrt{\epsilon}.
\%
Here the first inequality follows from Cauchy-Schwarz inequality and the second follows from the fact that $\sqrt{\bar{p}_{f_{\hat\theta}}(\bm{x}){p}_{f_{\hat\theta}}(\bm{x})}\geq{p}_{f_{\hat\theta}}(\bm{x})$. By \eqref{101508} and \eqref{101509}, we have
\%
1-\int\sqrt{{p}_{f_{\hat\theta}}(\bm{x})p_{f_{\theta^* }}(\bm{x})}\,d\bm{x}\leq \sqrt{\epsilon}+\frac{1}{m}\log\frac{N_{\b}\big(\mP(\mathcal{F}_{\theta}),\epsilon\big)}{\delta},
\%
which implies that
\%
H^2\big({p}_{f_{\hat\theta}}(\bm{x}),p_{f_{\theta^* }}(\bm{x})\big)=1-\int\sqrt{{p}_{f_{\hat\theta}}(\bm{x})p_{f_{\theta^* }}(\bm{x})}\,d\bm{x}\leq \sqrt{\epsilon}+\frac{1}{m}\log\frac{N_{\b}\big(\mP(\mathcal{F}_{\theta}),\epsilon\big)}{\delta}.
\%
Set $\epsilon=1/m^2$. We have
\%
H^2\big({p}_{f_{\hat\theta}}(x,x't),p_{f_{\theta^* }}(x,x',t)\big)\leq \frac{2}{m}\log\frac{N_{\b}\big(\mP(\mathcal{F}_{\theta}),1/m^2\big)}{\delta}.
\%



\end{proof}
